Bounded Model Checking of Multi-threaded Software using SMT solvers

The transition from single-core to multi-core processors has made multi-threaded software an important subject in computer aided verification. Here, we describe and evaluate an extension of the ESBMC model checker to support the verification of multi-threaded software with shared variables and locks using bounded model checking (BMC) based on Satisfiability Modulo Theories (SMT). We describe three approaches to model check multi-threaded software and our modelling of the synchronization primitives of the Pthread library. In the lazy approach, we generate all possible interleavings and call the BMC procedure on each of them individually, until we either find a bug, or have systematically explored all interleavings. In the schedule recording approach, we encode all possible interleavings into one single formula and then exploit the high speed of the SMT solvers. In the underapproximation-widening approach, we reduce the state space by abstracting the number of state variables and interleavings from the proofs of unsatisfiability generated by the SMT solvers. In all three approaches, we use partial-order reduction (POR) techniques to reduce the number of interleavings explored. Experiments show that our approaches can analyze larger problems and substantially reduce the verification time compared to state-of-the-art techniques that combine classic POR methods with symbolic algorithms and others that implement the Counter-Example Guided Abstraction Refinement technique.

==> 02-background.tex <==
%------------------------------------------------------
\section{SMT and Proofs of Unsatisfiability}
\label{02-ProofsofUnsatisfiability}
%------------------------------------------------------

SMT decides the satisfiability of first-order formulae using a combination of different background theories and thus generalizes propositional satisfiability by supporting uninterpreted functions, linear and non-linear arithmetic, bit-vectors, tuples, arrays, and other decidable first-order theories (for a complete survey about SMT, we refer the reader to~\cite{MouraB09}). SMT solvers use multi-sorted first-order terms~\cite{MouraB08}. Formulae are represented by terms of Boolean sort, and terms are represented by function application, bound variables, and quantification~\cite{MouraB08} (in this work, we are then concerned with the satisfiability problem of the \textbf{quantifier-free fragment} of a \textbf{theory} T that consists of a set of formulae without quantifiers). Proof objects are also represented as terms and are derived from axioms. A proof-tree is a term where each inference rule is represented by an interpreted and/or uninterpreted function. For example, the proof-rule for modus ponens can be represented as:

%
\begin{equation}
\label{modus-pones}
\frac{p \rightarrow q, p}{q}
\end{equation}

\noindent 






